On The Performance of ARM TrustZone

The TrustZone technology, available in the vast majority of recent ARM processors, allows the execution of code inside a so-called secure world. It effectively provides hardware-isolated areas of the processor for sensitive data and code, i.e., a trusted execution environment (TEE). The OP-TEE framework provides a collection of toolchain, open-source libraries and secure kernel specifically geared to develop applications for TrustZone. This paper presents an in-depth performance- and energy-wise study of TrustZone using the OP-TEE framework, including secure storage and the cost of switching between secure and unsecure worlds, using emulated and hardware measurements.

==> related_work.tex <==
% !TEX root = main.tex
\section{Related Work}\label{sec:relwork}
\vs{possible suggestions to fill this section. List papers that: make experimental evaluations of systems, study tradeoffs of existing technologies, use TrustZone (ICDCS'18, SRDS'18 - RK). Does not need to be extremely long, between half and 1 page.}

\subsection{GlobalPlatform}

GlobalPlatform\cite{globalplatform} is an association involving members from different industries which promotes and edictates APIs guidelines focused on the interoperability of secure applications across different hardware platforms.
Split in two main parts, namely the Client- and Internal- API, they describe the interfaces available in the secure world, to TAs, as well as how to create a context and establish a session with a TA.
Their specifications are complete as they specify the name of the function, its parameters, return value and a description of their goal. Additional structures required to use the interface are also described in detail.
The internal API has a wide coverage and offers many encryption, hashing and signing facilities.
OP-TEE complies with the GlobalPlatform's specifications and its implementation is used in this thesis.

\subsection{Qemu}

A relatively recent addition to the Qemu emulator\cite{qemu} was the support of the TrustZone extension enabling it to implement the normal/secure world paradigm.
This emulator is provided by OP-TEE and is used in this thesis.

\subsection{weaveOS}

weeveOS\cite{weeveos} is a lightweight open source operating system aiming to unite the currently fragmented IoT ecosystem.
It runs on off-the-shelf IoT boards supporting the ARM TrustZone extension.
The weeveOS offers facilities for secure data channels via MQTTS, trustworthy processing and data collection, and ensuring data integrity and trust by using a blockchain system.
A gateway assumes the role of message broker and handles all communication related tasks. It also provides health checks, secure device management, access control, accounting and key management.

